Testing Sparsity over Known and Unknown Bases

Sparsity is a basic property of real vectors that is exploited in a wide variety of applications. In this work, we describe property testing algorithms for sparsity that observe a low-dimensional projection of the input. We consider two settings. In the first setting, for a given design matrix A in R^{d x m}, we test whether an input vector y in R^d equals Ax for some k-sparse unit vector x. Our algorithm projects the input onto O(k \eps^{-2} log m) dimensions, accepts if the property holds, rejects if ||y - Ax|| > \eps for any O(k/\eps^2)-sparse vector x, and runs in time polynomial in m. Our algorithm is based on the approximate Caratheodory's theorem. Previously known algorithms that solve the problem for arbitrary A with qualitatively similar guarantees run in exponential time. In the second setting, the design matrix A is unknown. Given input vectors y_1, y_2,...,y_p in R^d whose concatenation as columns forms Y in R^{d x p} , the goal is to decide whether Y=AX for matrices A in R^{d x m} and X in R^{m x p} such that each column of X is k-sparse, or whether Y is "far" from having such a decomposition. We give such a testing algorithm which projects the input vectors to O(log p/\eps^2) dimensions and assumes that the unknown A satisfies k-restricted isometry. Our analysis gives a new robust characterization of gaussian width in terms of sparsity.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{array}
\usepackage{graphicx}
\usepackage{color}
\usepackage{calc}
%\usepackage{fontspec}
\usepackage{framed}
\usepackage[shortlabels]{enumitem}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{bbm}

%\setromanfont{Garamond}
%\setsansfont{Segoe UI}
%\setmonofont{Consolas}

\newcommand{\from}{\leftarrow}

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}

\newcommand{\bP}{\mathbb{P}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bF}{\mathbb{F}}


\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfp}{\mathbf{p}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cC}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

\newcommand{\sP}{\ensuremath{\mathsf{P}}}
\newcommand{\sNP}{\ensuremath{\mathsf{NP}}}

\newcommand{\problembreak}{\hfill $\blacksquare$}

% TODO: Define macros for probability, expectation.
\newcommand{\Prob}[1]{ \mathbf{P}\left( #1 \right) }
\newcommand{\Probx}[2]{ \mathrm{P}_{#1}\left( #2 \right) }
\newcommand{\prob}[1]{ \mathbf{p}\left( #1 \right) }
\newcommand{\Exp}[1]{ \bE\left[ #1 \right] }

\newcounter{lecnum}
\setcounter{lecnum}{3}
\newtheorem{definition}{Definition}[lecnum]
\newtheorem{claim}{Claim}[lecnum]
\newtheorem{lemma}{Lemma}[lecnum]
\newtheorem{proposition}{Proposition}[lecnum]
\newtheorem{theorem}{Theorem}[lecnum]
\newtheorem{conjecture}{Conjecture}[lecnum]
\newtheorem{corollary}{Corollary}[lecnum]

\setlength{\parindent}{0pt}
\setlength{\parskip}{10pt plus4pt minus2pt}

\newcommand{\abs}[1]{\ensuremath{\left| #1 \right|}}

\newcommand{\defproblem}[3]
{
	%\begin{table}[h!]	
	\begin{tabular}{|r p{\columnwidth-6.2em}|}
	\hline
	\multicolumn{2}{|c|}{ #1 } \\
	\hline
	\emph{Input:}		& #2 \\
	\emph{Question:}	& #3 \\
	\hline
	\end{tabular} \\
	%\end{table}
}


